A Carbon Tracking Model for Federated Learning: Impact of Quantization and Sparsification

Federated Learning (FL) methods adopt efficient communication technologies to distribute machine learning tasks across edge devices, reducing the overhead in terms of data storage and computational complexity compared to centralized solutions. Rather than moving large data volumes from producers (sensors, machines) to energy-hungry data centers, raising environmental concerns due to resource demands, FL provides an alternative solution to mitigate the energy demands of several learning tasks while enabling new Artificial Intelligence of Things (AIoT) applications. This paper proposes a framework for real-time monitoring of the energy and carbon footprint impacts of FL systems. The carbon tracking tool is evaluated for consensus (fully decentralized) and classical FL policies. For the first time, we present a quantitative evaluation of different computationally and communication efficient FL methods from the perspectives of energy consumption and carbon equivalent emissions, suggesting also general guidelines for energy-efficient design. Results indicate that consensus-driven FL implementations should be preferred for limiting carbon emissions when the energy efficiency of the communication is low (i.e., < 25 Kbit/Joule). Besides, quantization and sparsification operations are shown to strike a balance between learning performances and energy consumption, leading to sustainable FL designs.

==> Sections/Section2-old.tex <==
\section{Carbon tracking framework \label{sec:Energy-footprint-modeling}}

Energy and carbon footprint models in FL (see \cite{first_look,tgcn}
for a review) assume that the energy budget of the learning process
can be broken down into computing and communication costs. Notice
that both the PS ($k=0$), when used, and the learner/devices ($k>0$)
contribute to the energy balance, and their footprints should be evaluated
separately. The goal of this section is to revisit FL energy models
targeting the definition of a framework for the real-time tracking
of the carbon footprint. Let $\mathrm{C}_{k}(t)$ refer to the equivalent
GHG emissions of device $k$ observed at time $t\geq t_{0}$, with
$t_{0}$ being the starting time of the learning process, the proposed
carbon tracking tool quantifies the increased emissions at time $t+\triangle t$
($\triangle t\geq0$) through an iterative approach 
\begin{equation}
\mathrm{C}_{k}(t+\triangle t)=\int_{t}^{t+\triangle t}P_{k}(\tau)\cdot I_{k}(\tau)\cdot d\tau+\mathrm{C}_{k}(t)\label{eq:tracking_general}
\end{equation}
where $P_{k}(\tau)$ is power consumption of device $k$ at time $\tau$
and $I_{k}(\tau)$ is the corresponding carbon intensity of the electricity
generation \cite{LTE_power}, measured in Kg CO2-equivalent emissions
per kWh (KgCO2-eq/kWh). It quantifies how much carbon emissions are
produced per kilowatt hour of locally generated electricity. The $I_{k}(\tau)$
terms are typically monitored on hourly basis \cite{carbon_survey,pimrc}
as they depend on the specific regional energy grid where the devices
$k=0,...,K$ are installed. Notice that grid differences can result
in large variations in eq. CO2 emissions \cite{kone1}. In what follows,
we assume that a carbon tracking update is issued on every new FL
round. We therefore simplify (\ref{eq:tracking_general}) into 
\begin{equation}
\mathrm{C}_{k}(t_{i+1})=E_{k,i}\cdot I_{k}+\mathrm{C}_{k}(t_{i-1})\label{eq:tracking_general-1}
\end{equation}
where $E_{k,i}$ is the energy cost of FL round $i$ on device $k$
at time $t_{i+1}$. In the following, we model the energy cost $E_{k,i}$
based on the specific FL method employed. 

The communication costs are quantified on average, in terms of the
corresponding energy efficiencies ($\mathrm{EE}$), standardized by
ETSI (European Telecommunications Standards Institute \cite{ee_etsi}).
Efficiency terms in downlink (DL) $\mathrm{EE}_{\mathrm{D}}$, uplink
(UL) $\mathrm{EE}_{\mathrm{U}}$, or sidelink (S) $\mathrm{EE}_{\mathrm{S}}$
transmissions are measured here in bit/Joule {[}bit/J{]} \cite{ee}.
The efficiencies also include the power dissipated in the RF front-end,
conversion, baseband processing and other transceiver stages. 

\subsection{Energy tracking for Parameter Server based FL}

In vanilla FL methods, such as federated averaging, the PS collects
the local models produced by $K$ learners and produces a global model
of size $b_{\mathbf{W}}$ bits, which is fed back to active devices
on each round. Learners are powered on as they run the local optimizer
(LO) and decode the updated global model $\mathbf{W}_{i-1}$ obtained
from the PS at round $i-1$. During a single FL round, the energy
cost $E_{k,i} = E_{k,i}^{(\mathrm{FA})}$ of an individual learner
($k>0$) can be written as 
\begin{equation}
E_{k,i}^{(\mathrm{FA})}=E_{k,i}^{(\mathrm{C})}+\frac{b_{\mathbf{W}}}{\mathrm{EE}_{\mathrm{D}}}+\frac{\mathbb{Q}_{k,i}[b_{\mathbf{W}}]}{\mathrm{EE}_{\mathrm{U}}}+E_{k,\mathbb{Q}}^{(\mathrm{C})}+E_{k,\mathrm{sleep}}^{(\mathrm{C})},\label{eq:fagen}
\end{equation}
namely, the superposition of the energy spent for receiving the global
model from the PS $\frac{b_{\mathbf{W}}}{\mathrm{EE}_{\mathrm{D}}}$,
the cost for LO at round $i$, $E_{k,i}^{(\mathrm{C})}$ {[}Joule{]},
i.e., required for SGD computation, and the UL communication $\frac{\mathbb{Q}_{k}[b_{\mathbf{W}}]}{\mathrm{EE}_{\mathrm{U}}}$
of the selected local model parameters according to the model selection
and quantization policy $\mathbb{Q}_{k}[\cdot]$ (see Sect. 3). Implementation
of policy $\mathbb{Q}_{k}[\cdot]$ has a cost which is quantified here
as $E_{k,\mathbb{Q}}^{(\mathrm{C})}$. Finally, $E_{k,\mathrm{sleep}}^{(\mathrm{C})}$
is the energy cost in sleep mode, which is required by devices for
waiting for the global model to be produced by the PS. The PS ($k=0$)
energy per round is 
\begin{equation}
E_{0,i}^{(\mathrm{PS})}=K\cdot E_{0,\mathrm{global}}^{(\mathrm{C})}+\frac{b_{\mathbf{W}}}{\mathrm{EE}_{\mathrm{U}}}+\sum_{k=1}^{K}\frac{\mathbb{Q}_{k,i}[b_{\mathbf{W}}]}{\mathrm{EE}_{\mathrm{D}}}+E_{0,\mathrm{sleep}}^{(\mathrm{C})},
\end{equation}
it accounts for the cost for $K$ global model updates $E_{0,\mathrm{global}}^{(\mathrm{C})}$,
global model DL publication $\frac{b_{\mathbf{W}}}{\mathrm{EE}_{\mathrm{U}}},$and
collection of local model parameters $\frac{\mathbb{Q}_{k,i}[b_{\mathbf{W}}]}{\mathrm{EE}_{\mathrm{D}}}$
from the $K$ learners.
\textcolor{black}{The total carbon emissions produced under the FA scheme can be evaluated as 
\begin{equation}
    \mathrm{C}_{\text{tot}}^{\text{(FA)}} = \sum_{i} \sum_{k = 1}^{N} \mathrm{C}_k^{(\text{FA})}(t_{i}) + \sum_{i} \mathrm{C}^{(\text{PS})}_0(t_{i})
\end{equation}
where $\mathrm{C}^{(\text{FA})}_k(t_{i}) = E_{k,i}^{\text{(FA)}} \cdot I_{k} + \mathrm{C}_k^{(\text{FA})}(t_{i-1})$ is the carbon footprint of device $k$ at round $i$ while $\mathrm{C}_0^{(\text{PS})}(t_{i}) = E_{0,i}^{\text{(PS)}} \cdot I_{0} + \mathrm{C}_0^{(\text{PS})}(t_{i-1})$ is the carbon footprint of the PS at round $i$.}
 

\subsection{Energy tracking for decentralized and consensus-driven FL}

Decentralized FL techniques \cite{chen,commmag} do not employ the
PS as the learners mutually exchange their local model parameters,
i.e., through publish-subscribe operations \cite{access}. Each learner
is responsible of producing a global model representation which is
the result of a consensus over the received local model parameters
obtained from neighbor learners. In what follows we adopt a distributed
weighted averaging approach \cite{commmag,chen} used to combine the
received neighbor models, referred to as CFA. As shown in Fig. \ref{fig:cfa_vs_fa},
the learners/devices mutually exchange their local model parameters
with an assigned number $N<K$ of neighbors.

Let $\mathcal{N}_{k,i}$ be the set that contains the $N$ chosen
neighbors of node $k$ at round $i$, the energy cost $E_{k,i}=E_{k,i}^{(\mathrm{CFA})}$
of an individual learner ($k>0$) can be written as 
\begin{equation}
\begin{aligned}E_{k,i}^{(\mathrm{CFA})}={} & E_{k,i}^{(\mathrm{C})}+N\cdot E_{k,\mathrm{global}}^{(\mathrm{C})}+\sum_{h\in\mathcal{N}_{k,i}}\frac{\mathbb{Q}_{h,i}[b_{\mathbf{W}}]}{\mathrm{EE}_{\mathrm{S}}}\\
{} & +\frac{\mathbb{Q}_{k,i}[b_{\mathbf{W}}]}{\mathrm{EE}_{\mathrm{S}}}+E_{k,\mathbb{Q}}^{(\mathrm{C})}+E_{k,\mathrm{sleep}}^{(\mathrm{C})},
\end{aligned}
\label{eq:cfa}
\end{equation}
where now each learner should implement the LO, $E_{k,i}^{(\mathrm{C})}$,
produce a global model representation via $N$ weighted averaging
steps $E_{k,\mathrm{global}}^{(\mathrm{C})}$, distribute the local
(selected) parameters and obtain the neighbor ones using sidelink
communications. Notice that, when the sidelink interface is not available,
communication among the learners could be implemented by UL and DL
communications: therefore $[\mathrm{EE}_{\mathrm{S}}]^{-1}\simeq[\mathrm{EE}_{\mathrm{D}}]^{-1}+[\mathrm{EE}_{\mathrm{U}}]^{-1}$.
\textcolor{black}{Finally, the total carbon consumption under the CFA scheme can be quantified as
\begin{equation}
\mathrm{C}_{\text{tot}}^{\text{(CFA)}} = \sum_{i}  \sum_{k = 1}^{N} \mathrm{C}^{(\text{CFA})}_k(t_{i})
\end{equation}
with $C_k^{(\text{CFA})}(t_{i}) = E_{k,i}^{(\text{CFA})} \cdot I_k + C_k^{(\text{CFA})}(t_{i-1})$ being the carbon footprint of device $k$ at round $i$.}








==> Sections/Section3_old.tex <==
\section{Quantization and parameter selection in FL}

This section presents the compression strategies employed for evaluating the impact of the communication on the energy/carbon footprint for the proposed FL setups.
To guarantee a fair comparison, we assume that both centralized and decentralized FL tools rely on the same compression operators.
More specifically, we consider two widely-adopted mechanisms, namely top-$t$ sparsification \cite{topk} and probabilistic quantization \cite{qsgd}, which are applied independently by each device member of the federation.

Given a generic input vector $\mathbf{v}$ that may represent the model parameters or some surrogate quantities, the compression policy aims at obtaining a lower bit representation of such vector by successively applying sparsification and quantization as  
\begin{equation}
\bar{\mathbf{v}} = \mathcal{Q}(\mathbf{v}) = f_q(f_s(\mathbf{v})) , 
\label{eq:generic_quantization}
\end{equation}
where $\mathcal{Q}(.)$ denotes the overall compression function, while $f_s(.)$ and $f_q(.)$ indicate the operators required for top-$t$ sparsification and probabilistic quantization, respectively. 
In particular, $f_s(.)$ outputs a new representation $\widetilde{\mathbf{v}} = f_s(\mathbf{v})$ by selecting the $t$ entries with the largest absolute values and sets all other entries to 0. 
On the other hand, $f_q(.)$ encodes $\widetilde{\mathbf{v}}$ via a randomized rounding operation.
The quantizer operates on each entry $\widetilde{v}_{n}$ of $\widetilde{\mathbf{v}}$, with $n = 1, \ldots, N_{P}$ where $N_{P}$ denotes the number of elements of $\widetilde{\mathbf{v}}$, and is defined as \cite{qsgd} 
\begin{equation}
\bar{v}_{n} = \|\widetilde{\mathbf{v}} \|_2 \cdot \mathrm{sign}(\widetilde{v}_{n}) \xi_{n} (\widetilde{\mathbf{v}}, 2^{N_b}) ,
%\ f_p(\mathrm{clip}(|\widetilde{p}_{k,i,n}|, 2^{}), N_{b}) , 
\end{equation}
where $\mathrm{sign}(.)$ denotes the sign operator, $N_b$ the number of bits, while 
\begin{equation}
\xi_{n} (\widetilde{\mathbf{v}}, 2^{N_b}) = \begin{cases}
\ell/N_{\ell} & \text{with probability} \\
& 1- \frac{|\widetilde{v}_{n}|}{\|\widetilde{\mathbf{v}} \|_2} N_{\ell} - \ell \\ %p\left(\frac{|\widetilde{p}_{k,i,n}|}{\|\widetilde{\mathbf{P}}_{k,i} \|_2}, N_{\ell}\right)\\
(\ell +1)/N_{\ell} & \text{otherwise} ,\\
\end{cases}
\end{equation}
where $0 \leq \ell \leq N_{\ell}$ and $N_{\ell} = 2^{N_b} -1$ is the number of quantization levels.
Finally, each quantized entry is collected in the vector  
\begin{equation}
\bar{\mathbf{v}} = [\bar{v}_{1}, \ldots, \bar{v}_{N_{P}}]^{\mathrm{T}} ,
\end{equation}   
and can be used as a lower bit representation of $\mathbf{v}$. 
In what follows, we review the specific operations required for implementing the considered compression strategies for the vanilla FL (Sec. \ref{subsec:compression_vanilla_FL}) and the consensus-driven FL (Sec. \ref{subsec:compression_consensus_FL}) schemes.   


\subsection{Parameter Server based FL}
\label{subsec:compression_vanilla_FL}

In vanilla FL, the devices send to the PS the model updates as they are more suited for compression \cite{compr_fl}. 
Given the model parameters $\mathbf{W}_{k,i}$ of device $k$ at round $i$, the model updates are evaluated as
\begin{equation}
\mathbf{P}_{k,i} = \mathbf{W}_{k,i+1/2} - \mathbf{W}_{k,i} ,
\label{eq:model_update}
\end{equation} where $\mathbf{W}_{k,i+1/2}$ denotes the model parameters obtained after LO for device $k$ at round $i$. 
Then, $\mathbf{P}_{k,i}$ is compressed as
\begin{equation}
\bar{\mathbf{P}}_{k,i} = \mathcal{Q}(\mathbf{P}_{k,i})
\label{eq:compressed_model_update}
\end{equation} 
with $\mathcal{Q}(.)$ as in \eqref{eq:generic_quantization}
and the resulting vector is exchanged with the PS.
The PS updates its global model by aggregating the contributions received by the devices as 
\begin{equation}
\mathbf{W}_{t+1} = \mathbf{W}_{t} + \sum_{k = 1}^{N} \sigma_{k} \bar{\mathbf{P}}_{k,i}
\end{equation}
where $\sigma_{k}$ is a weighting factor.
Finally, the PS shares the updated global model with the devices and a new learning round starts. 
Note that the PS forwards back the updated model uncompressed as highlighted in Sec. \ref{sec:Energy-footprint-modeling}.
Considering the aforementioned compression policies, each device is required to forward $\mathbb{Q}_{k,i}[b_{\mathbf{W}}]$ bits that can be quantified as 
\begin{equation}
\mathbb{Q}_{k,i}[b_{\mathbf{W}}] =\dfrac{t}{N_{P}} \dfrac{N_{bc}}{N_b} b_{\mathbf{W}} ,
\label{eq:bits_used}
\end{equation}
where $N_{bc}$ is a typical value used for encoding the model parameters in most deep learning frameworks (e.g., 32 bits).	


\subsection{Decentralized FL based on CHOCO-SGD framework} 
\label{subsec:compression_consensus_FL}


The consensus-driven FL process considered here relies on the CHOCO-SGD algorithm proposed in \cite{gossipc}. 
This scheme employs two additional variables at each device to track and compensate for the compression errors over consecutive learning rounds. 
In the same spirit as the centralized FL tool, each device $k$ compresses the model updates in a manner similar to \eqref{eq:model_update}-\eqref{eq:compressed_model_update} leading to 
\begin{equation}
\bar{\mathbf{P}}_{k,i} = \mathcal{Q}(\mathbf{P}_{k,i}) = \mathcal{Q}(\mathbf{W}_{k,i+1/2} - \mathbf{X}_{k,i})
\label{eq:model_updates_consensus} ,
\end{equation}
where $\mathcal{Q}(.)$ is defined as in \eqref{eq:generic_quantization}
and $\mathbf{X}_{k,i}$ is a local variable used for keeping track the compression errors related to its local model.
Then, $\bar{\mathbf{P}}_{k,i}$ is exchanged over the network and $\mathbf{X}_{k,i}$ is updated as
\begin{equation}
\mathbf{X}_{k,i+1} = \mathbf{X}_{k,i} + \bar{\mathbf{P}}_{k,i} .
\end{equation}
The devices receiving the contributions from their neighbors update their local model as  
\begin{equation}
\mathbf{W}_{k,i+1} = \mathbf{W}_{k,i} + \gamma (\mathbf{S}_{k,i+1} - \mathbf{X}_{k,i+1}) ,
\end{equation}
where $\gamma$ is the consensus step-size, while 
\begin{equation}
\mathbf{S}_{k,i+1} = \mathbf{S}_{k,i} + \sum_{j \in \mathcal{N}_{k,i}} \omega_{k,j} \bar{\mathbf{P}}_{j,i} ,
\end{equation}
where $\omega_{k,j}$ is the $(k,j)$-th entry of a symmetric doubly stochastic matrix $\boldsymbol{\Omega}$, while $\mathbf{S}_{k,i}$ is a local variable stored at each device $k$ and is used to keep track of the compression errors of the neighbors of device $k$ over consecutive learning rounds.   
Note that at round $i = 0$, the local variables are set as $\mathbf{X}_{k,0} = \mathbf{S}_{k,0} = \mathbf{0}$. 
Similarly as in Sec. \ref{subsec:compression_vanilla_FL}, each device uses the same number of bits $\mathbb{Q}_{k,i}[b_{\mathbf{W}}]$ defined in \eqref{eq:bits_used} for transmitting the model updates in \eqref{eq:model_updates_consensus}.

%- Qui le strategie communication efficient: 1) metodo statico (quantizzazione classica fix su tutto il modello e vedere se fare round-robin sparisfier), 2) dinamico (quantizzazione fissa con parameter selection)
%e adaptive (solo quantizzazione adattativa) e hybrid (parameter selection basato su gradiente).
